The minimum rank problem over the finite field of order 2: minimum rank 3

Our main result is a sharp bound for the number of vertices in a minimal forbidden subgraph for the graphs having minimum rank at most 3 over the finite field of order 2. We also list all 62 such minimal forbidden subgraphs. We conclude by exploring how some of these results over the finite field of order 2 extend to arbitrary fields and demonstrate that at least one third of the 62 are minimal forbidden subgraphs over an arbitrary field for the class of graphs having minimum rank at most 3 in that field.

==> graphs/Makefile <==
# Make the .tex files for each graph for graphs 1-62.

graphs: forbiddengraphs.pic graphmacros.pic
	for i in `seq 1 62`; do printf "specialchars\ngraph%d\n.PE\n"  $$i| cat forbiddengraphs.pic - | dpic -e > graph-$$i.tex; done;
	for i in P3cartP2minusvertex k3vpk3 k3vpk3vpk1 graph38inline graph38deleteinline graph39inline graph39_inside graph39_outside graph39_outside_pendant graph40_pendant graph44_pendant; do printf "\nscale=pts/8;circlerad=.75/pts*scale;\nlinethick=.4;\n%s\n.PE\n" $$i | cat othergraphs.pic - | dpic -e > $$i.tex; done;
	for i in graph39_v; do printf "\nscale=1.5;circlerad=.1*scale;\n%s\n.PE\n" $$i | cat othergraphs.pic - | dpic -e > $$i.tex; done;
	for i in threek2 dart fullhouse ltimes P3UK2 P3VP3 P3cartP2 P3 P4 threeprism examplea exampleb; do printf "%s\n.PE\n" $$i | cat othergraphs.pic - | dpic -e > $$i.tex; done;
	for i in p4nottight; do printf "scale=1.7;circlerad=.05*scale\n%s\n.PE\n" $$i | cat othergraphs.pic - | dpic -e > $$i.tex; done;
#	for i in *.tex; do sed  -i "" -e "s/0\.4pt/0\.5pt/g" -e "s/0\.8pt/0\.7pt/g" $$i; done;
clean: 
	for ((i=1;i<=62;i++)); do rm `printf "graph-%d.tex"  $$i`; done;
	for i in k3vpk3 k3vpk3vpk1 graph38inline graph38deleteinline graph39inline graph39_inside graph39_outside graph39_outside_pendant graph40_pendant graph44_pendant; do rm `printf "%s.tex"  $$i`; done;
	for i in graph39_v; do rm `printf "%s.tex"  $$i`; done; 
	for i in threek2 dart fullhouse ltimes P3UK2 P3VP3 P4 threeprism p4nottight ; do rm `printf "%s.tex"  $$i`; done;

# To generate the tabbing envir nment laying out these graphs, 
# 4 on a line, just do:
# for ((i=1,j=2,k=3,h=4;i<=62;i+=4,j+=4,k+=4,h+=4)); do printf "\input graphs/graph-%d.tex \> \input graphs/graph-%d.tex \> \input graphs/graph-%d.tex \> \input graphs/graph-%d.tex \\\\\\\\\n" $i $j $k $h; done;

# Then change the first line's "\>" to "\=", delete any extraneous
# \inputs at the end of the list, and copy into a tabbing environment
# in your paper.

